Leveraging Neural Radiance Fields for Uncertainty-Aware Visual Localization

As a promising fashion for visual localization, scene coordinate regression (SCR) has seen tremendous progress in the past decade. Most recent methods usually adopt neural networks to learn the mapping from image pixels to 3D scene coordinates, which requires a vast amount of annotated training data. We propose to leverage Neural Radiance Fields (NeRF) to generate training samples for SCR. Despite NeRF's efficiency in rendering, many of the rendered data are polluted by artifacts or only contain minimal information gain, which can hinder the regression accuracy or bring unnecessary computational costs with redundant data. These challenges are addressed in three folds in this paper: (1) A NeRF is designed to separately predict uncertainties for the rendered color and depth images, which reveal data reliability at the pixel level. (2) SCR is formulated as deep evidential learning with epistemic uncertainty, which is used to evaluate information gain and scene coordinate quality. (3) Based on the three arts of uncertainties, a novel view selection policy is formed that significantly improves data efficiency. Experiments on public datasets demonstrate that our method could select the samples that bring the most information gain and promote the performance with the highest efficiency.

==> figures/more_uncertainty.tex <==
\begin{figure*}[ht]
% \setlength{\abovecaptionskip}{0.4cm}
% \setlength{\belowcaptionskip}{-0.3cm}
    \centering
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000794.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000794.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000794.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000794.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000794.depth_to16b_std_vis.png}
     \end{subfigure}  
    \\[0.2ex]

     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000021.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000021.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000021.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000021.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000021.depth_to16b_std_vis.png}
     \end{subfigure}  
    \\[0.2ex]

     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000651.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000651.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000651.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000651.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000651.depth_to16b_std_vis.png}
     \end{subfigure}  
    \\[0.2ex]

     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000878.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000878.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000878.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000878.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000878.depth_to16b_std_vis.png}
     \end{subfigure}  
    \\[0.2ex]

     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001106.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001106.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001106.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001106.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001106.depth_to16b_std_vis.png}
     \end{subfigure}  
    \\[0.2ex]

     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001146.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001146.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001146.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001146.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001146.depth_to16b_std_vis.png}
     \end{subfigure}  
    \\[0.2ex]

    %  \begin{subfigure}[b]{0.19\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000614.resize_color.jpg}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.19\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000614.rgb_error_map_vis.png}
    %  \end{subfigure}
    % \begin{subfigure}[b]{0.19\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000614.rgb_to16b_std_vis.png}
    %  \end{subfigure}
    % \begin{subfigure}[b]{0.19\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000614.depth_error_map.png}
    %  \end{subfigure}
    % \begin{subfigure}[b]{0.19\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000614.depth_to16b_std_vis.png}
    %  \end{subfigure}  
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001070.resize_color.jpg}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001070.rgb_error_map_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001070.rgb_to16b_std_vis.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001070.depth_error_map.png}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-001070.depth_to16b_std_vis.png}
     \end{subfigure}   
    \\[0.2ex]

     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000052.resize_color.jpg}
         \caption{Rendered RGB}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000052.rgb_error_map_vis.png}
         \caption{Color prediction error}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000052.rgb_to16b_std_vis.png}
         \caption{Color uncertainty}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000052.depth_error_map.png}
         \caption{Depth prediction error}
     \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/uncertainty_maps/frame-000052.depth_to16b_std_vis.png}
         \caption{Depth uncertainty}
     \end{subfigure}     
     
    \caption[uncertainty]{Additional qualitative results of U-NeRF uncertainty estimation.}
    \label{fig:more_uncertainty}
\end{figure*}

==> figures/pcd_filter.tex <==
% \vspace{-0.5cm}
\begin{figure}[ht]
\setlength{\abovecaptionskip}{0.3cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
% \includegraphics[width=\textwidth]{images/depth_filter/render00_crop2.png}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/depth_filter/filter01_crop2.png}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/depth_filter/real02_crop2.png} 
%      \end{subfigure}
%      \\[0.2ex]
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/depth_filter/render.png}
         \caption{Rendered}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/depth_filter/filtered.png}
         \caption{Filtered}
     \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/depth_filter/real.png}
         \caption{Ground truth}
     \end{subfigure}
    \caption[filter]{Removing noisy regions using NeRF uncertainty.}
    \label{fig:pcd_filter}
\end{figure}

==> figures/rendered_rgb_compare.tex <==
\begin{figure*}[ht]
% \setlength{\abovecaptionskip}{0.4cm}
% \setlength{\belowcaptionskip}{-0.3cm}
    \centering

     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/active-frame-001147.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/nerfw-frame-001147.resize_color.jpg} 
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/our-frame-001147.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}      
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/gt-frame-001147.color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}  
    \\[2ex]
    
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/active-frame-000076.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/nerfw-frame-000076.resize_color.jpg} 
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/our-frame-000076.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}      
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/gt-frame-000076.color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}  
    \\[2ex]

     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/active-frame-000391.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/nerfw-frame-000391.resize_color.jpg} 
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/our-frame-000391.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}      
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/gt-frame-000391.color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}  
    \\[2ex]

     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/active-frame-001178.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/nerfw-frame-001178.resize_color.jpg} 
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/our-frame-001178.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}      
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/gt-frame-001178.color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}  
    \\[2ex]

     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/active-frame-000100.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/nerfw-frame-000100.resize_color.jpg} 
         \captionsetup{labelformat=empty}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/our-frame-000100.resize_color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}      
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/gt-frame-000100.color.jpg}
         \captionsetup{labelformat=empty}
     \end{subfigure}  
    \\[2ex]

     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/active-frame-001031.resize_color.jpg}
         \captionsetup{labelformat=empty}
         \caption{ActiveNeRF~\cite{pan2022activenerf}}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/nerfw-frame-001031.resize_color.jpg} 
         \captionsetup{labelformat=empty}
         \caption{NeRF-W~\cite{martin2021nerf}}
     \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/our-frame-001031.resize_color.jpg}
         \captionsetup{labelformat=empty}
         \caption{Ours}
     \end{subfigure}      
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ms_images/nerf/gt-frame-001031.color.jpg}
         \captionsetup{labelformat=empty}
         \caption{Ground truth}
     \end{subfigure}  
    \\[2ex]
    
    \caption[rendered rgb]{Qualitative results of rendered RGB images.}
    \label{fig:rendered_rgb_compare}
\end{figure*}

==> figures/zeta_nll.tex <==
\begin{figure}[ht]
\setlength{\abovecaptionskip}{0.4cm}
\setlength{\belowcaptionskip}{-0.4cm}
    \centering
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
% \includegraphics[width=\textwidth]{images/nerf/rgb_681_no_ue_mark2.png}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/nerf/rgb_681_mark2.png}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/nerf/target_rgb_681_mark2.png} 
%      \end{subfigure}
%      \\[0.2ex]
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/nerf/rgb_681_no_ue_crop.png}
         \caption{NLL}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/nerf/rgb_681_crop.png}
         \caption{$\zeta$-NLL}
     \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/nerf/target_rgb_681_crop.png}
         \caption{Ground truth}
     \end{subfigure}
    \caption[zeta nll]{NLL vs $\zeta$-NLL}
    \label{fig:zeta_nll}
\end{figure}

==> tables/12scenes.tex <==

\begin{table*}[]
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
% \normalsize
% \small
% \setlength\tabcolsep{3.6pt}
\footnotesize
\setlength\tabcolsep{5pt}
% \begin{tabular}{c|ccc|ccc|ccc|cc|cc}
% \hline
% \multirow{2}{*}{\textbf{Scene}} & \multicolumn{3}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \multicolumn{3}{c|}{\textbf{Ours (+120 novel views)}} & \multicolumn{3}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \multicolumn{2}{c|}{\textbf{DSAC++}} & \multicolumn{2}{c}{\textbf{HSCNet}} \\
%                                 & Imgs        & Acc.        & Med.             & Imgs     & Acc.    & Med.          & Imgs      & Acc.      & Med.           & Acc.              & Med.             & Acc.          & Med.                \\ \hline
% living-1                        & 176         & 92.6        & 0.024, 0.8       & 296      & 97.6    & 0.021, 0.6    & 1035      & 100       & 0.011, 0.4     & 100               & -                & 100           & 0.011, 0.4          \\
% living-2                        & 169         & 61.8        & 0.042, 1.8       & 289      & 95.1    & 0.020, 0.8    & 731       & 100       & 0.014, 0.6     & 100               & -                & 100           & 0.010, 0.4          \\
% luke                            & 197         & 58.6        & 0.044, 1.4       & 317      & 90.0    & 0.026, 1.0    & 1370      & 93.8      & 0.020, 0.9     & 95.5              & -                & 96.3          & 0.012, 0.5          \\
% gates362                        & 190         & 88.6        & 0.026, 0.8       & 310      &         &               & 3540      & 100       & 0.011, 0.5     & 100               & -                & 100           & 0.010, 0.4          \\
% gates381                        & 193         & 76.3        & 0.034, 1.4       & 313      & 81.4    & 0.027, 1.2    & 2950      & 98.8      & 0.016, 0.7     & 96.8              & -                & 99.1          & 0.012, 0.6          \\
% 5a                              & 178         & 65.9        & 0.036, 1.5       & 298      & 80.3    & 0.025, 0.9    & 1001      & 97.0      & 0.016, 0.7     & 83.7              & -                & 98.8          & 0.012, 0.5          \\ \hline
% \end{tabular}


% \begin{tabular}{c|ccccc|ccccccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{5}{c|}{\textbf{Few views training}}                                                                 & \multicolumn{7}{c}{\textbf{All views training}}                                                                                                    \\ \cline{2-13} 
%                                 & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \multicolumn{2}{c|}{\textbf{SCRNet-EDL (Ours)}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \multicolumn{2}{c|}{\textbf{DSAC++~\cite{brachmann2018learning}}} & \multicolumn{2}{c}{\textbf{HSCNet~\cite{li2020hierarchical}}} \\ \cline{2-13} 
%                                 & \multicolumn{1}{c|}{Imgs}      & Acc. & \multicolumn{1}{c|}{Med.}     & Acc.              & Med.                 & \multicolumn{1}{c|}{Imgs}      & Acc. & \multicolumn{1}{c|}{Med.}     & Acc.   & \multicolumn{1}{c|}{Med.}   & Acc.           & Med.               \\ \hline
% living-1                        & \multicolumn{1}{c|}{176}       & 92.6 & \multicolumn{1}{c|}{2.4, 0.8} & 97.6              & 2.1, 0.6             & \multicolumn{1}{c|}{1035}      & 100  & \multicolumn{1}{c|}{1.1, 0.4} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.1, 0.4           \\
% living-2                        & \multicolumn{1}{c|}{169}       & 61.8 & \multicolumn{1}{c|}{4.2, 1.8} & 95.1              & 2.0, 0.8             & \multicolumn{1}{c|}{731}       & 100  & \multicolumn{1}{c|}{1.4, 0.6} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
% luke                            & \multicolumn{1}{c|}{197}       & 58.6 & \multicolumn{1}{c|}{4.4, 1.4} & 90.0              & 2.6, 1.0             & \multicolumn{1}{c|}{1370}      & 93.8 & \multicolumn{1}{c|}{2.0, 0.9} & 95.5   & \multicolumn{1}{c|}{-}      & 96.3           & 1.2, 0.5           \\
% gates362                        & \multicolumn{1}{c|}{190}       & 88.6 & \multicolumn{1}{c|}{2.6, 0.8} & 91.0              & 2.0, 0.8             & \multicolumn{1}{c|}{3540}      & 100  & \multicolumn{1}{c|}{1.1, 0.5} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
% gates381                        & \multicolumn{1}{c|}{193}       & 76.3 & \multicolumn{1}{c|}{3.4, 1.4} & 81.4              & 2.7, 1.2             & \multicolumn{1}{c|}{2950}      & 98.8 & \multicolumn{1}{c|}{1.6, 0.7} & 96.8   & \multicolumn{1}{c|}{-}      & 99.1           & 1.2, 0.6           \\
% 5a                              & \multicolumn{1}{c|}{178}       & 65.9 & \multicolumn{1}{c|}{3.6, 1.5} & 80.3              & 2.5, 0.9             & \multicolumn{1}{c|}{1001}      & 97.0 & \multicolumn{1}{c|}{1.6, 0.7} & 83.7   & \multicolumn{1}{c|}{-}      & 98.8           & 1.2, 0.5           \\ \hline
% \end{tabular}
% \caption{Visual localization results on 12-Scenes dataset. We report median pose error in (cm,\degree), and percentages of error \textless5cm, 5\degree.}
% \label{tab:12s_result}
% \end{table*}


% Please add the following required packages to your document preamble:
% \begin{tabular}{c|ccccc|ccccccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{5}{c|}{\textbf{Few views training}}                                                                 & \multicolumn{7}{c}{\textbf{All views training}}                                                                                                    \\ \cline{2-13} 
%                                 & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{SCRNet}} & \multicolumn{2}{c|}{\textbf{SCRNet-EDL}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{SCRNet}} & \multicolumn{2}{c|}{\textbf{DSAC++}} & \multicolumn{2}{c}{\textbf{HSCNet}} \\ \cline{2-13} 
%                                 & \multicolumn{1}{c|}{Imgs}      & Acc. & \multicolumn{1}{c|}{Med.}     & Acc.              & Med.                 & \multicolumn{1}{c|}{Imgs}      & Acc. & \multicolumn{1}{c|}{Med.}     & Acc.   & \multicolumn{1}{c|}{Med.}   & Acc.           & Med.               \\ \hline
% kitchen-1                       & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                   &                      & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &        & \multicolumn{1}{c|}{}       &                &                    \\
% living-1                        & \multicolumn{1}{c|}{176}       & 92.6 & \multicolumn{1}{c|}{2.4, 0.8} & 97.6              & 2.1, 0.6             & \multicolumn{1}{c|}{1035}      & 100  & \multicolumn{1}{c|}{1.1, 0.4} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.1, 0.4           \\
% Bed                             & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                   &                      & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &        & \multicolumn{1}{c|}{}       &                &                    \\
% kitchen-2                       & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                   &                      & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &        & \multicolumn{1}{c|}{}       &                &                    \\
% living-2                        & \multicolumn{1}{c|}{169}       & 61.8 & \multicolumn{1}{c|}{4.2, 1.8} & 95.1              & 2.0, 0.8             & \multicolumn{1}{c|}{731}       & 100  & \multicolumn{1}{c|}{1.4, 0.6} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
% luke                            & \multicolumn{1}{c|}{197}       & 58.6 & \multicolumn{1}{c|}{4.4, 1.4} & 90.0              & 2.6, 1.0             & \multicolumn{1}{c|}{1370}      & 93.8 & \multicolumn{1}{c|}{2.0, 0.9} & 95.5   & \multicolumn{1}{c|}{-}      & 96.3           & 1.2, 0.5           \\
% gates362                        & \multicolumn{1}{c|}{190}       & 88.6 & \multicolumn{1}{c|}{2.6, 0.8} & 91.0              & 2.0, 0.8             & \multicolumn{1}{c|}{3540}      & 100  & \multicolumn{1}{c|}{1.1, 0.5} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
% gates381                        & \multicolumn{1}{c|}{193}       & 76.3 & \multicolumn{1}{c|}{3.4, 1.4} & 81.4              & 2.7, 1.2             & \multicolumn{1}{c|}{2950}      & 98.8 & \multicolumn{1}{c|}{1.6, 0.7} & 96.8   & \multicolumn{1}{c|}{-}      & 99.1           & 1.2, 0.6           \\
% lounge                          & \multicolumn{1}{c|}{}          & 86.9 & \multicolumn{1}{c|}{2.7, 0.9} & 97.0              & 1.8, 0.6             & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &        & \multicolumn{1}{c|}{}       &                &                    \\
% manolis                         & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                   &                      & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &        & \multicolumn{1}{c|}{}       &                &                    \\
% 5a                              & \multicolumn{1}{c|}{178}       & 65.9 & \multicolumn{1}{c|}{3.6, 1.5} & 80.3              & 2.5, 0.9             & \multicolumn{1}{c|}{1001}      & 97.0 & \multicolumn{1}{c|}{1.6, 0.7} & 83.7   & \multicolumn{1}{c|}{-}      & 98.8           & 1.2, 0.5           \\
% 5b                              & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                   &                      & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &        & \multicolumn{1}{c|}{}       &                &                    \\ \hline
% \end{tabular}

% \begin{tabular}{c|cccllcc|ccccccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{7}{c|}{\textbf{Few views training}}                                                                                                                  & \multicolumn{7}{c}{\textbf{All views training}}                                                                                                    \\ \cline{2-15} 
%                                 & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{SCRNet}} & \multicolumn{2}{c|}{\textbf{SCRNet-ID}}              & \multicolumn{2}{c|}{\textbf{Ours}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{SCRNet}} & \multicolumn{2}{c|}{\textbf{DSAC++}} & \multicolumn{2}{c}{\textbf{HSCNet}} \\ \cline{2-15} 
%                                 & \multicolumn{1}{c|}{Imgs}      & Acc. & \multicolumn{1}{c|}{Med.}     & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c|}{Med.} & Acc.           & Med.              & \multicolumn{1}{c|}{Imgs}      & Acc. & \multicolumn{1}{c|}{Med.}     & Acc.   & \multicolumn{1}{c|}{Med.}   & Acc.           & Med.               \\ \hline
% kitchen-1                       & \multicolumn{1}{c|}{150}       &      & \multicolumn{1}{c|}{}         &                          & \multicolumn{1}{l|}{}     & 100            & 0.9, 0.5          & \multicolumn{1}{c|}{744}       & 100  & \multicolumn{1}{c|}{0.8, 0.4} & 100    & \multicolumn{1}{c|}{-}      & 100            & 0.8, 0.4           \\
% living-1                        & \multicolumn{1}{c|}{176}       & 92.6 & \multicolumn{1}{c|}{2.4, 0.8} &                          & \multicolumn{1}{l|}{}     & 97.6           & 2.1, 0.6          & \multicolumn{1}{c|}{1035}      & 100  & \multicolumn{1}{c|}{1.1, 0.4} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.1, 0.4           \\
% Bed                             & \multicolumn{1}{c|}{143}       &      & \multicolumn{1}{c|}{}         &                          & \multicolumn{1}{l|}{}     &                &                   & \multicolumn{1}{c|}{894}       & 100  & \multicolumn{1}{c|}{1.3, 0.6} & 99.5   & \multicolumn{1}{c|}{-}      & 100            & 0.9, 0.4           \\
% kitchen-2                       & \multicolumn{1}{c|}{156}       &      & \multicolumn{1}{c|}{}         &                          & \multicolumn{1}{l|}{}     &                &                   & \multicolumn{1}{c|}{782}       & 100  & \multicolumn{1}{c|}{0.8, 0.4} & 99.5   & \multicolumn{1}{c|}{-}      & 100            & 0.7, 0.3           \\
% living-2                        & \multicolumn{1}{c|}{169}       & 61.8 & \multicolumn{1}{c|}{4.2, 1.8} &                          & \multicolumn{1}{l|}{}     & 95.1           & 2.0, 0.8          & \multicolumn{1}{c|}{731}       & 100  & \multicolumn{1}{c|}{1.4, 0.6} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
% luke                            & \multicolumn{1}{c|}{197}       & 58.6 & \multicolumn{1}{c|}{4.4, 1.4} &                          & \multicolumn{1}{l|}{}     & 90.0           & 2.6, 1.0          & \multicolumn{1}{c|}{1370}      & 93.8 & \multicolumn{1}{c|}{2.0, 0.9} & 95.5   & \multicolumn{1}{c|}{-}      & 96.3           & 1.2, 0.5           \\
% gates362                        & \multicolumn{1}{c|}{190}       & 88.6 & \multicolumn{1}{c|}{2.6, 0.8} &                          & \multicolumn{1}{l|}{}     & 91.0           & 2.0, 0.8          & \multicolumn{1}{c|}{3540}      & 100  & \multicolumn{1}{c|}{1.1, 0.5} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
% gates381                        & \multicolumn{1}{c|}{193}       & 76.3 & \multicolumn{1}{c|}{3.4, 1.4} &                          & \multicolumn{1}{l|}{}     & 81.4           & 2.7, 1.2          & \multicolumn{1}{c|}{2950}      & 98.8 & \multicolumn{1}{c|}{1.6, 0.7} & 96.8   & \multicolumn{1}{c|}{-}      & 99.1           & 1.2, 0.6           \\
% lounge                          & \multicolumn{1}{c|}{170}       & 86.9 & \multicolumn{1}{c|}{2.7, 0.9} &                          & \multicolumn{1}{l|}{}     & 97.0           & 1.8, 0.6          & \multicolumn{1}{c|}{933}       & 99.4 & \multicolumn{1}{c|}{1.5, 0.5} & 95.1   & \multicolumn{1}{c|}{-}      & 100            & 1.4, 0.5           \\
% manolis                         & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                          & \multicolumn{1}{l|}{}     &                &                   & \multicolumn{1}{c|}{1623}      & 97.2 & \multicolumn{1}{c|}{1.4, 0.7} & 96.4   & \multicolumn{1}{c|}{-}      & 100            & 1.1, 0.5           \\
% 5a                              & \multicolumn{1}{c|}{178}       & 65.9 & \multicolumn{1}{c|}{3.6, 1.5} &                          & \multicolumn{1}{l|}{}     & 80.3           & 2.5, 0.9          & \multicolumn{1}{c|}{1001}      & 97.0 & \multicolumn{1}{c|}{1.6, 0.7} & 83.7   & \multicolumn{1}{c|}{-}      & 98.8           & 1.2, 0.5           \\
% 5b                              & \multicolumn{1}{c|}{}          &      & \multicolumn{1}{c|}{}         &                          & \multicolumn{1}{l|}{}     &                &                   & \multicolumn{1}{c|}{1441}      & 93.3 & \multicolumn{1}{c|}{1.9, 0.6} & 95.0   & \multicolumn{1}{c|}{-}      & 97.3           & 1.5, 0.5           \\ \hline
% \end{tabular}
% \caption{Visual localization results on 12-Scenes dataset. We report median pose error in (cm,$\degree$), and percentages of error \textless5cm, 5$\degree$.}

\begin{tabular}{c|ccccccc|ccccccc}
\hline
\multirow{3}{*}{\textbf{Scene}} & \multicolumn{7}{c|}{\textbf{Few views training}}                                                                                                     & \multicolumn{7}{c}{\textbf{All views training}}                                                                                                    \\ \cline{2-15} 
                                & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{SCRNet~\cite{li2020hierarchical}} & \multicolumn{2}{c|}{SCRNet-ID~\cite{ng2021reassessing}} & \multicolumn{2}{c|}{Ours} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{SCRNet~\cite{li2020hierarchical}} & \multicolumn{2}{c|}{DSAC++~\cite{brachmann2018learning}} & \multicolumn{2}{c}{HSCNet~\cite{li2020hierarchical}} \\ \cline{2-15} 
                                & \multicolumn{1}{c|}{Images}      & Acc.$\uparrow$ & \multicolumn{1}{c|}{Med.$\downarrow$}     & Acc.$\uparrow$   & \multicolumn{1}{c|}{Med.$\downarrow$}      & Acc.$\uparrow$           & Med.$\downarrow$              & \multicolumn{1}{c|}{Images}      & Acc.$\uparrow$ & \multicolumn{1}{c|}{Med.$\downarrow$}     & Acc.$\uparrow$   & \multicolumn{1}{c|}{Med.$\downarrow$}   & Acc.$\uparrow$           & Med.$\downarrow$               \\ \hline
kitchen-1                       & \multicolumn{1}{c|}{150}       & 90.4 & \multicolumn{1}{c|}{2.3, 1.3} & 87.1   & \multicolumn{1}{c|}{2.6, 1.4}  & \textbf{100}   & \textbf{0.9, 0.5} & \multicolumn{1}{c|}{744}       & 100  & \multicolumn{1}{c|}{0.8, 0.4} & 100    & \multicolumn{1}{c|}{-}      & 100            & 0.8, 0.4           \\
living-1                        & \multicolumn{1}{c|}{176}       & 92.6 & \multicolumn{1}{c|}{2.4, 0.8} & 91.4   & \multicolumn{1}{c|}{\textbf{2.0}, 0.8}  & \textbf{97.6}  & 2.1, \textbf{0.6}          & \multicolumn{1}{c|}{1035}      & 100  & \multicolumn{1}{c|}{1.1, 0.4} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.1, 0.4           \\
Bed                             & \multicolumn{1}{c|}{143}       & 73.5 & \multicolumn{1}{c|}{3.3, 1.5} & 82.3   & \multicolumn{1}{c|}{2.0, 0.8}  & \textbf{97.5}  & \textbf{1.6, 0.7} & \multicolumn{1}{c|}{894}       & 100  & \multicolumn{1}{c|}{1.3, 0.6} & 99.5   & \multicolumn{1}{c|}{-}      & 100            & 0.9, 0.4           \\
kitchen-2                       & \multicolumn{1}{c|}{156}       & 88.5 & \multicolumn{1}{c|}{2.1, 1.0} & 90.5   & \multicolumn{1}{c|}{1.8, 0.9}  & \textbf{97.1}  & \textbf{1.2, 0.5} & \multicolumn{1}{c|}{782}       & 100  & \multicolumn{1}{c|}{0.8, 0.4} & 99.5   & \multicolumn{1}{c|}{-}      & 100            & 0.7, 0.3           \\
living-2                        & \multicolumn{1}{c|}{169}       & 61.8 & \multicolumn{1}{c|}{4.2, 1.8} & 79.9   & \multicolumn{1}{c|}{3.0, 1.2}  & \textbf{95.1}  & \textbf{2.0, 0.8} & \multicolumn{1}{c|}{731}       & 100  & \multicolumn{1}{c|}{1.4, 0.6} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
luke                            & \multicolumn{1}{c|}{197}       & 58.6 & \multicolumn{1}{c|}{4.4, 1.4} & 73.3   & \multicolumn{1}{c|}{3.7, 1.3}  & \textbf{90.0}  & \textbf{2.6, 1.0} & \multicolumn{1}{c|}{1370}      & 93.8 & \multicolumn{1}{c|}{2.0, 0.9} & 95.5   & \multicolumn{1}{c|}{-}      & 96.3           & 1.2, 0.5           \\
gates362                        & \multicolumn{1}{c|}{190}       & 88.6 & \multicolumn{1}{c|}{2.6, \textbf{0.8}} & 87.6   & \multicolumn{1}{c|}{2.1, 1.0}  & \textbf{91.0}  & \textbf{2.0, 0.8} & \multicolumn{1}{c|}{3540}      & 100  & \multicolumn{1}{c|}{1.1, 0.5} & 100    & \multicolumn{1}{c|}{-}      & 100            & 1.0, 0.4           \\
gates381                        & \multicolumn{1}{c|}{193}       & 76.3 & \multicolumn{1}{c|}{3.4, 1.4} & \textbf{82.8}   & \multicolumn{1}{c|}{2.9, \textbf{1.2}}  & 81.4           & \textbf{2.7, 1.2} & \multicolumn{1}{c|}{2950}      & 98.8 & \multicolumn{1}{c|}{1.6, 0.7} & 96.8   & \multicolumn{1}{c|}{-}      & 99.1           & 1.2, 0.6           \\
lounge                          & \multicolumn{1}{c|}{170}       & 86.9 & \multicolumn{1}{c|}{2.7, 0.9} & 78.9   & \multicolumn{1}{c|}{3.4, 1.1}  & \textbf{97.0}  & \textbf{1.8, 0.6} & \multicolumn{1}{c|}{933}       & 99.4 & \multicolumn{1}{c|}{1.5, 0.5} & 95.1   & \multicolumn{1}{c|}{-}      & 100            & 1.4, 0.5           \\
manolis                         & \multicolumn{1}{c|}{241}       & 84.0 & \multicolumn{1}{c|}{1.8, 1.0} & 85.3   & \multicolumn{1}{c|}{2.6, 1.2}  & \textbf{94.1}  & \textbf{1.6, 0.7} & \multicolumn{1}{c|}{1623}      & 97.2 & \multicolumn{1}{c|}{1.4, 0.7} & 96.4   & \multicolumn{1}{c|}{-}      & 100            & 1.1, 0.5           \\
5a                              & \multicolumn{1}{c|}{178}       & 65.9 & \multicolumn{1}{c|}{3.6, 1.5} & 72.8   & \multicolumn{1}{c|}{3.3, 1.2}  & \textbf{80.3}  & \textbf{2.5, 0.9} & \multicolumn{1}{c|}{1001}      & 97.0 & \multicolumn{1}{c|}{1.6, 0.7} & 83.7   & \multicolumn{1}{c|}{-}      & 98.8           & 1.2, 0.5           \\
5b                              & \multicolumn{1}{c|}{228}       & 64.7 & \multicolumn{1}{c|}{3.4, 1.2} & 66.7   & \multicolumn{1}{c|}{3.8, 1.3}  & \textbf{81.5}  & \textbf{2.6, 0.8} & \multicolumn{1}{c|}{1441}      & 93.3 & \multicolumn{1}{c|}{1.9, 0.6} & 95.0   & \multicolumn{1}{c|}{-}      & 97.3           & 1.5, 0.5           \\ \hline
\end{tabular}
\caption{Visual localization results on 12-Scenes. We report median translation and rotation errors (cm,\degree). We also report accuracy as the percentages of error \textless5cm, 5\degree. The best results under the few views training are labeled in bold.}
\label{tab:12s_result}
\end{table*}




==> tables/12scenes_few.tex <==
\begin{table}[]
\footnotesize
\setlength\tabcolsep{2.4pt}
\begin{tabular}{c|cc|cc|cc|cc}
\hline
          & \multicolumn{2}{c|}{SCRNet}       & \multicolumn{2}{c|}{SCRNet-ID}                    & \multicolumn{2}{c|}{SRC}          & \multicolumn{2}{c}{Ours}                                            \\ \cline{2-9} 
          & Acc.$\uparrow$ & Med.$\downarrow$ & Acc.$\uparrow$                 & Med.$\downarrow$ & Acc.$\uparrow$ & Med.$\downarrow$ & Acc.$\uparrow$                 & Med.$\downarrow$                   \\ \hline
kitchen-1 & 90.4           & 2.3, 1.3         & 87.1                           & 2.6, 1.4         &                &                  & \textbf{100}  & \textbf{0.9, 0.5} \\
living-1  & 92.6           & 2.4, 0.8         & 91.4                           & 2.0, 0.8         &                &                  & \textbf{97.6} & 2.1, \textbf{0.6} \\
Bed       & 73.5           & 3.3, 1.5         & 82.3                           & 2.0, 0.8         &                &                  & \textbf{97.5} & \textbf{1.6, 0.7} \\
kitchen-2 & 88.5           & 2.1, 1.0         & 90.5                           & 1.8, 0.9         &                &                  & \textbf{97.1} & \textbf{1.2, 0.5} \\
living-2  & 61.8           & 4.2, 1.8         & 79.9                           & 3.0, 1.2         &                &                  & \textbf{95.1} & \textbf{2.0, 0.8} \\
luke      & 58.6           & 4.4, 1.4         & 73.3                           & 3.7, 1.3         &                &                  & \textbf{90.0} & \textbf{2.6, 1.0} \\
gates362  & 88.6           & 2.6, 0.8         & 87.6                           & 2.1, 1.0         &                &                  & \textbf{91.0} & \textbf{2.0, 0.8} \\
gates381  & 76.3           & 3.4, 1.4         & \textbf{82.8} & 2.9, 1.2         &                &                  & 81.4                           & \textbf{2.7, 1.2} \\
lounge    & 86.9           & 2.7, 0.9         & 78.9                           & 3.4, 1.1         &                &                  & \textbf{97.0} & \textbf{1.8, 0.6} \\
manolis   & 84.0           & 1.8, 1.0         & 85.3                           & 2.6, 1.2         &                &                  & \textbf{94.1} & \textbf{1.6, 0.7} \\
5a        & 65.9           & 3.6, 1.5         & 72.8                           & 3.3, 1.2         &                &                  & \textbf{80.3} & \textbf{2.5, 0.9} \\
5b        & 64.7           & 3.4, 1.2         & 66.7                           & 3.8, 1.3         &                &                  & \textbf{81.5} & \textbf{2.6, 0.8} \\ \hline
\end{tabular}
\caption{Visual localization results on 12-Scenes. We report median translation and rotation errors (cm,\degree). We also report accuracy as the percentages of error \textless5cm, 5\degree. The best results under the few views training are labeled in bold.}
\label{tab:12s_result}
\end{table}

==> tables/7scenes.tex <==

% \begin{table}[]
% \setlength{\abovecaptionskip}{0.2cm}
% % \setlength{\belowcaptionskip}{-0.5cm}
% \centering
% % \normalsize
% % \small
% \footnotesize
% \setlength\tabcolsep{2pt}
% \begin{tabular}{c|cccc|cccl}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{4}{c|}{\textbf{Few views training}}                                   & \multicolumn{4}{c}{\textbf{All views training}}                            \\ \cline{2-9} 
%                                 & \multicolumn{2}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}}          & \multicolumn{2}{c|}{\textbf{Ours}} & \multicolumn{2}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \multicolumn{2}{c}{\textbf{DSAC++~\cite{brachmann2018learning}}} \\ \cline{2-9} 
%                                 & Acc.$\uparrow$          & \multicolumn{1}{c|}{Med.$\downarrow$}     & Acc.$\uparrow$           & Med.$\downarrow$              & Acc.$\uparrow$  & \multicolumn{1}{c|}{Med.$\downarrow$}    & Acc.$\uparrow$   & \multicolumn{1}{c}{Med.$\downarrow$}   \\ \hline
% chess                           & 78.1          & \multicolumn{1}{c|}{3.0, 1.1} & \textbf{80.2}  & \textbf{2.7, 0.9} & 95.4  & \multicolumn{1}{c|}{2, 0.7}  & 97.1   & 2, 0.5                     \\
% fire                            & 75.9          & \multicolumn{1}{c|}{3.4, 1.4} & \textbf{85.3}  & \textbf{2.6, 1.1} & 94.9  & \multicolumn{1}{c|}{2, 0.9}  & 89.6   & 2, 0.9                     \\
% heads                           & \textbf{97.8} & \multicolumn{1}{c|}{1.4, \textbf{0.9}} & 97.0           & \textbf{1.3}, 1.0          & 97.1  & \multicolumn{1}{c|}{1, 0.8}  & 92.4   & 1, 0.8                     \\
% office                          & 59.0          & \multicolumn{1}{c|}{4.3, 1.2} & \textbf{63.8}  & \textbf{3.8, 1.1} & 81.4  & \multicolumn{1}{c|}{3, 0.9}  & 86.6   & 3, 0.7                     \\
% pumpkin                         & 44.9          & \multicolumn{1}{c|}{5.4, \textbf{1.3}} & \textbf{47.3}  & \textbf{5.2, 1.3} & 58.0  & \multicolumn{1}{c|}{4, 1.1}  & 59.0   & 4, 1.1                     \\
% redkitchen                      & 31.6          & \multicolumn{1}{c|}{7.1, 2.0} & \textbf{31.7}  & \textbf{7.0, 1.9} & 56.5  & \multicolumn{1}{c|}{5, 1.4}  & 66.6   & 4, 1.1                     \\
% stairs                          & 43.3          & \multicolumn{1}{c|}{5.5, 1.5} & \textbf{61.3}  & \textbf{4.5, 1.1} & 68.1  & \multicolumn{1}{c|}{4, 1.0}  & 29.3   & 9, 2.6                     \\ \hline
% \end{tabular}
% \caption{Visual localization results on 7-Scenes~\cite{shotton2013scene}. We report median translation and rotation errors (cm,\degree), and accuracy as the percentages of error \textless5cm, 5\degree. The best results under the few views training are labeled in bold.}
% \label{tab:7s_result}
% \end{table}


\begin{table}[]
\footnotesize
\setlength\tabcolsep{2pt}
\begin{tabular}{c|cc|cc|cc|cc}
\hline
           & \multicolumn{2}{c|}{SCRNet}                       & \multicolumn{2}{c|}{SCRNet-ID}                                             & \multicolumn{2}{c|}{SRC}                                                   & \multicolumn{2}{c}{Ours}                                            \\ \cline{2-9} 
           & Acc.$\uparrow$                 & Med.$\downarrow$ & \multicolumn{1}{c}{Acc.$\uparrow$} & \multicolumn{1}{c|}{Med.$\downarrow$} & \multicolumn{1}{c}{Acc.$\uparrow$} & \multicolumn{1}{c|}{Med.$\downarrow$} & Acc.$\uparrow$                 & Med.$\downarrow$                   \\ \hline
chess      & 78.1                           & 3.0, 1.1         & 76.1                               & 3.1, 1.1                              & 77.5                               & 3.6, 1.1                              & \textbf{80.2} & \textbf{2.7, 0.9} \\
fire       & 75.9                           & 3.4, 1.4         & 74.1                               & 3.3, 1.3                              &  -                                  &   -                                    & \textbf{85.3} & \textbf{2.6, 1.1} \\
heads      & 97.8 & 1.4, \textbf{0.9}         & 96.0                               & 1.4, 1.1                              & \textbf{99.0}                               & 1.8, 1.2                              & 97.0                           & \textbf{1.3}, 1.0 \\
office     & 59.0                           & 4.3, 1.2         & 45.2                               & 5.5, 1.5                              & 42.3                               & 5.6, 1.4                              & \textbf{63.8} & \textbf{3.8, 1.1} \\
pumpkin    & 44.9                           & 5.4, 1.3         & 43.0                               & 5.6, 1.3                              & 42.0                               & 5.8, 1.5                              & \textbf{47.3} & \textbf{5.2, 1.3} \\
redkitchen & 31.6                           & 7.1, 2.0         & 33.5                               & 7.0, 2.1                              & 25.6                               & 6.9, \textbf{1.8}                              & \textbf{34.8} & \textbf{6.8}, 1.9 \\
stairs     & 43.3                           & 5.5, 1.5         & 50.9                               & 4.9, 1.3                              & 48.2                               & 5.1, 1.4                              & \textbf{61.3} & \textbf{4.5, 1.1} \\ \hline
\end{tabular}
\caption{Visual localization results on 7-Scenes~\cite{shotton2013scene}. We report median translation and rotation errors (cm,\degree), and accuracy as the percentages of error \textless5cm, 5\degree. The best results under the few views training are labeled in bold.}
\label{tab:7s_result}
\end{table}

==> tables/7scenes_and_cambridge.tex <==
\begin{table*}[]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.4cm}
\footnotesize
\setlength\tabcolsep{2.3pt}
\begin{tabular}{c|ccccc|ccccc|c|cc|cc}
\hline
\multirow{3}{*}{\textbf{7-Scenes}} & \multicolumn{5}{c|}{\textbf{Few views training}}                                                               & \multicolumn{5}{c|}{\textbf{All views training}}                                                        & \multirow{3}{*}{\textbf{Cambridge}} & \multicolumn{2}{c|}{\textbf{Few views training}}        & \multicolumn{2}{c}{\textbf{All views training}}       \\ \cline{2-11} \cline{13-16} 
                                   & \multicolumn{1}{c|}{}     & \multicolumn{2}{c|}{SCRNet~\cite{li2020hierarchical}}          & \multicolumn{2}{c|}{Ours} & \multicolumn{1}{c|}{}     & \multicolumn{2}{c|}{SCRNet~\cite{li2020hierarchical}} & \multicolumn{2}{c|}{DSAC++~\cite{brachmann2018learning}} &                                     & \multicolumn{1}{c|}{SCRNet~\cite{li2020hierarchical}} & Ours$^\dagger$    & \multicolumn{1}{c|}{SCRNet~\cite{li2020hierarchical}} & DSAC$\ast$~\cite{brachmann2021dsacstar} \\ \cline{2-11} \cline{13-16} 
                                   & \multicolumn{1}{c|}{Images} & Acc.$\uparrow$          & \multicolumn{1}{c|}{Med.$\downarrow$}     & Acc.$\uparrow$           & Med.$\downarrow$              & \multicolumn{1}{c|}{Images} & Acc.$\uparrow$  & \multicolumn{1}{c|}{Med.$\downarrow$}    & Acc.$\uparrow$             & Med.$\downarrow$              &                                     & \multicolumn{1}{c|}{Med.$\downarrow$}            & Med.$\downarrow$             & \multicolumn{1}{c|}{Med.$\downarrow$}            & Med.$\downarrow$           \\ \hline
chess                              & \multicolumn{1}{c|}{250}  & 78.1          & \multicolumn{1}{c|}{3.0, 1.1} & \textbf{80.2}  & \textbf{2.7, 0.9} & \multicolumn{1}{c|}{4000} & 95.4  & \multicolumn{1}{c|}{2, 0.7}  & 97.1             & 2, 0.5            & Court                          & \multicolumn{1}{c|}{122, 0.7}        & \textbf{86, 0.5} & \multicolumn{1}{c|}{125, 0.6}        & 49, 0.3        \\
fire                               & \multicolumn{1}{c|}{250}  & 75.9          & \multicolumn{1}{c|}{3.4, 1.4} & \textbf{85.3}  & \textbf{2.6, 1.1} & \multicolumn{1}{c|}{2000} & 94.9  & \multicolumn{1}{c|}{2, 0.9}  & 89.6             & 2, 0.9            & College                        & \multicolumn{1}{c|}{27, 0.4}         & \textbf{23, 0.3} & \multicolumn{1}{c|}{21, 0.3}         & 15, 0.3        \\
heads                              & \multicolumn{1}{c|}{250}  & \textbf{97.8} & \multicolumn{1}{c|}{1.4, \textbf{0.9}} & 97.0           & \textbf{1.3}, 1.0          & \multicolumn{1}{c|}{1000} & 97.1  & \multicolumn{1}{c|}{1, 0.8}  & 92.4             & 1, 0.8            & Hospital                         & \multicolumn{1}{c|}{22, 0.4}         & \textbf{21, 0.3} & \multicolumn{1}{c|}{21, 0.3}         & 21, 0.4        \\
office                             & \multicolumn{1}{c|}{250}  & 59.0          & \multicolumn{1}{c|}{4.3, 1.2} & \textbf{63.8}  & \textbf{3.8, 1.1} & \multicolumn{1}{c|}{6000} & 81.4  & \multicolumn{1}{c|}{3, 0.9}  & 86.6             & 3, 0.7            & Shop                          & \multicolumn{1}{c|}{9, 0.4}          & \textbf{6, 0.3}  & \multicolumn{1}{c|}{6, 0.3}          & 5, 0.3         \\
pumpkin                            & \multicolumn{1}{c|}{250}  & 44.9          & \multicolumn{1}{c|}{5.4, 1.3} & \textbf{47.3}  & \textbf{5.2, 1.3} & \multicolumn{1}{c|}{4000} & 58.0  & \multicolumn{1}{c|}{4, 1.1}  & 59.0             & 4, 1.1            & Church                       & \multicolumn{1}{c|}{32, 0.8}         & \textbf{21, 0.6} & \multicolumn{1}{c|}{16, 0.5}         & 13, 0.4        \\
redkitchen                         & \multicolumn{1}{c|}{250}  & 31.6          & \multicolumn{1}{c|}{7.1, 2.0} & \textbf{34.8}  & \textbf{6.8, 1.9} & \multicolumn{1}{c|}{7000} & 56.5  & \multicolumn{1}{c|}{5, 1.4}  & 66.6             & 4, 1.1            & -                                   & \multicolumn{1}{c|}{-}               & -                & \multicolumn{1}{c|}{-}               & -              \\
stairs                             & \multicolumn{1}{c|}{250}  & 43.3          & \multicolumn{1}{c|}{5.5, 1.5} & \textbf{61.3}  & \textbf{4.5, 1.1} & \multicolumn{1}{c|}{2000} & 68.1  & \multicolumn{1}{c|}{4, 1.0}  & 29.3             & 9, 2.6            & -                                   & \multicolumn{1}{c|}{-}               & -       & \multicolumn{1}{c|}{-}               & -              \\ \hline
\end{tabular}
\caption{Visual localization results on 7-Scenes and Cambridge landmarks. We report median translation and rotation errors (cm,\degree), and accuracy as the percentages of error \textless5cm, 5\degree. The best results under the few views training are labeled in bold. Ours$^\dagger$ denotes E-SCRNet trained only using the initial real images $S_{real}$.}
\label{tab:7s_cambridge_results}
\end{table*}

==> tables/cambridge.tex <==

\begin{table}[]
\setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{-0.5cm}
\centering
% \normalsize
% \small
% \setlength\tabcolsep{3pt}
\footnotesize
\setlength\tabcolsep{2.6pt}
% \begin{tabular}{c|cc|cc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{2}{c|}{\textbf{Few views training}}          & \multicolumn{2}{c}{\textbf{All views training}}        \\ \cline{2-5} 
%                                 & \multicolumn{1}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \textbf{Ours}      & \multicolumn{1}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \textbf{DSAC++~\cite{brachmann2018learning}} \\ \cline{2-5} 
%                                 & \multicolumn{1}{c|}{Med.$\downarrow$}            & Med.$\downarrow$               & \multicolumn{1}{c|}{Med.$\downarrow$}            & Med.$\downarrow$            \\ \hline
% GreatCourt                      & \multicolumn{1}{c|}{1.22, 0.7}       & \textbf{0.86, 0.5} & \multicolumn{1}{c|}{1.25, 0.6}       & 0.40, 0.2       \\
% KingsCollege                    & \multicolumn{1}{c|}{0.27, 0.4}       & \textbf{0.23, 0.3} & \multicolumn{1}{c|}{0.21, 0.3}       & 0.18, 0.3       \\
% OldHospital                     & \multicolumn{1}{c|}{0.22, 0.4}       & \textbf{0.21, 0.3} & \multicolumn{1}{c|}{0.21, 0.3}       & 0.20, 0.3       \\
% ShopFacade                      & \multicolumn{1}{c|}{0.09, 0.4}       & \textbf{0.06, 0.3} & \multicolumn{1}{c|}{0.06, 0.3}       & 0.06, 0.3       \\
% StMarysChurch                   & \multicolumn{1}{c|}{0.32, 0.8}       & \textbf{0.21, 0.6} & \multicolumn{1}{c|}{0.16, 0.5}       & 0.13, 0.4       \\ \hline
% \end{tabular}
% 
\begin{tabular}{c|cc|cc}
\hline
\multirow{3}{*}{\textbf{Scene}} & \multicolumn{2}{c|}{\textbf{Few views training}}          & \multicolumn{2}{c}{\textbf{All views training}}        \\ \cline{2-5} 
                                & \multicolumn{1}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \textbf{E-SCRNet}      & \multicolumn{1}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}} & \textbf{DSAC*~\cite{brachmann2021dsacstar}} \\ \cline{2-5} 
                                & \multicolumn{1}{c|}{Med.$\downarrow$}            & Med.$\downarrow$               & \multicolumn{1}{c|}{Med.$\downarrow$}            & Med.$\downarrow$            \\ \hline
GreatCourt                      & \multicolumn{1}{c|}{1.22, 0.7}       & \textbf{0.86, 0.5} & \multicolumn{1}{c|}{1.25, 0.6}       & 0.49, 0.3       \\
KingsCollege                    & \multicolumn{1}{c|}{0.27, 0.4}       & \textbf{0.23, 0.3} & \multicolumn{1}{c|}{0.21, 0.3}       & 0.15, 0.3       \\
OldHospital                     & \multicolumn{1}{c|}{0.22, 0.4}       & \textbf{0.21, 0.3} & \multicolumn{1}{c|}{0.21, 0.3}       & 0.21, 0.4       \\
ShopFacade                      & \multicolumn{1}{c|}{0.09, 0.4}       & \textbf{0.06, 0.3} & \multicolumn{1}{c|}{0.06, 0.3}       & 0.05, 0.3       \\
StMarysChurch                   & \multicolumn{1}{c|}{0.32, 0.8}       & \textbf{0.21, 0.6} & \multicolumn{1}{c|}{0.16, 0.5}       & 0.13, 0.4       \\ \hline
\end{tabular}
\caption{Visual localization results on Cambridge~\cite{kendall2015posenet}. We report median translation and rotation errors (cm,\degree), and accuracy as the percentages of error \textless5cm, 5\degree. The best results under the few views training are labeled in bold.}
\label{tab:cambridge_result}
\end{table}

==> tables/compare_rgb_loss.tex <==
\begin{table}[]
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
\centering
\small
\setlength\tabcolsep{5pt}
\begin{tabular}{ccccc}
\hline
\textbf{Method} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{Depth RMSE$\downarrow$} \\ \hline
MSE~\cite{roessle2022dense} & 25.886    & 0.7409    & 0.3183    & \textbf{0.0199}    \\
NLL~\cite{pan2022activenerf} & 27.718    & 0.7527    & 0.3304    & 0.1064    \\
$\zeta$-NLL    & \textbf{28.741}    & \textbf{0.7819}    & \textbf{0.2823}    & 0.0227    \\ \hline
\end{tabular}
\caption{Comparing different RGB losses on kitchen-1.}
\label{tab:rgb_loss}
\end{table}

==> tables/replica_policy.tex <==
\begin{table}[h]
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.6cm}
\centering
\small
\setlength\tabcolsep{5.1pt}
\begin{tabular}{ccccc}
\hline
\textbf{Scene}           & \textbf{Policy} & \textbf{Median$\downarrow$} & \textbf{Mean$\downarrow$} & \textbf{Dist.$\downarrow$} \\ \hline
\multirow{2}{*}{room\_0} & Low score       & 2.07, 0.315     & 2.15, 0.322   & 0.232          \\
                         & High score      & 1.53, 0.243     & 1.98, 0.270   & 0.219          \\ \hline
\multirow{2}{*}{room\_1} & Low score       & 2.17, 0.346     & 2.47, 0.418   & 0.191          \\
                         & High score      & 1.96, 0.312     & 2.19, 0.389   & 0.173          \\ \hline
\multirow{2}{*}{room\_2} & Low score       & 1.64, 0.291     & 3.04, 0.671   & 0.387          \\
                         & High score      & 1.34, 0.220     & 2.57, 0.557   & 0.302          \\ \hline
\end{tabular}
\caption{Effectiveness of novel views selection policy.}
\label{tab:replica_policy}
\end{table}

==> tables/replica_table.tex <==
% \begin{table*}[]
% \setlength{\abovecaptionskip}{0.2cm}
% % \setlength{\belowcaptionskip}{-0.5cm}
% \centering
% % \small
% \footnotesize
% \setlength\tabcolsep{2.6pt}
% \begin{tabular}{c|cccccccc|ccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{8}{c|}{\textbf{Few views training}}                                                                                                                                                        & \multicolumn{3}{c}{\textbf{All views training}}           \\ \cline{2-12} 
%                                 & \multicolumn{3}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}}                                & \multicolumn{3}{c|}{\textbf{SCRNet-EDL (Ours)}}                            & \multicolumn{2}{c|}{\textbf{SRC~\cite{dong2022visual}}}     & \multicolumn{3}{c}{\textbf{SCRNet~\cite{li2020hierarchical}}}        \\ \cline{2-12} 
%                                 & Med.$\downarrow$ & Mean$\downarrow$ & \multicolumn{1}{c|}{Dist.$\downarrow$} & Med.$\downarrow$ & Mean$\downarrow$ & \multicolumn{1}{c|}{Dist.$\downarrow$} & Med.$\downarrow$ & Mean$\downarrow$ & Med.$\downarrow$ & Mean$\downarrow$ & Dist.$\downarrow$ \\ \hline
% room\_0                         & 2.05, \textcolor{blue}{0.33}         & 2.38, \textcolor{blue}{0.36}       & \multicolumn{1}{c|}{0.27}              & \textcolor{red}{1.53, 0.24}         & \textcolor{red}{1.98, 0.27}       & \multicolumn{1}{c|}{\textcolor{red}{0.22}}              & 2.78, 0.54         & 3.11, 0.64       & \textcolor{blue}{1.84}, 0.38         & \textcolor{blue}{2.05}, 0.39       & \textcolor{blue}{0.25}              \\
% room\_1                         & \textcolor{red}{1.84}, 0.34         & 2.21, 0.42       & \multicolumn{1}{c|}{0.21}              & 1.96,\textcolor{blue}{0.31}         & \textcolor{blue}{2.19, 0.38}       & \multicolumn{1}{c|}{\textcolor{red}{0.17}}              & \textcolor{blue}{1.92}, 0.35         & 3.40, 0.74       & 1.99, \textcolor{red}{0.30}         & \textcolor{red}{2.18, 0.35}       & \textcolor{blue}{0.18}              \\
% room\_2                         & \textcolor{red}{1.31},\textcolor{blue}{0.26}         & 2.69, 0.65       & \multicolumn{1}{c|}{0.37}              & 1.34, \textcolor{red}{0.22}         & \textcolor{blue}{2.57, 0.55}       & \multicolumn{1}{c|}{\textcolor{red}{0.30}}              & 2.97, 0.63         & 13.03, 3.44      & 1.58, 0.31         & \textcolor{red}{2.04, 0.49}       & \textcolor{blue}{0.35}              \\
% office\_0                       & 1.69,\textcolor{blue}{0.34}         & 2.01, 0.45       & \multicolumn{1}{c|}{0.17}              & \textcolor{blue}{1.61}, 0.35         & 1.97, 0.44       & \multicolumn{1}{c|}{\textcolor{red}{0.15}}              & \textcolor{red}{1.45, 0.30}         & \textcolor{blue}{1.92, 0.43}       & 1.85, 0.36         & \textcolor{red}{1.90, 0.42}       & \textcolor{red}{0.15}              \\
% office\_1                       & 2.10, 0.52         & 2.23, 0.63       & \multicolumn{1}{c|}{0.34}              & \textcolor{blue}{1.54, 0.44}         & \textcolor{blue}{1.74, 0.53}       & \multicolumn{1}{c|}{\textcolor{red}{0.22}}              & 2.07, 0.53         & 2.22, 0.59       & \textcolor{red}{1.46, 0.37}         & \textcolor{red}{1.70, 0.45}       & \textcolor{blue}{0.30}              \\
% office\_2                       & \textcolor{blue}{2.21, 0.41}         & \textcolor{blue}{2.54}, 0.49       & \multicolumn{1}{c|}{0.29}              & \textcolor{red}{1.69, 0.33}         & \textcolor{red}{1.93, 0.37}       & \multicolumn{1}{c|}{\textcolor{red}{0.25}}              & 2.53, 0.51         & 3.20, 0.64       & 2.79, 0.43         & 2.91, \textcolor{blue}{0.44}       & \textcolor{blue}{0.28}              \\
% office\_3                       & \textcolor{red}{2.13}, \textcolor{blue}{0.37}         & 4.91, 0.94       & \multicolumn{1}{c|}{0.44}              & 2.40, 0.38         & \textcolor{blue}{4.25, 0.86}       & \multicolumn{1}{c|}{\textcolor{red}{0.36}}              & 3.44, 0.63         & 21.52, 7.95      & \textcolor{blue}{2.16}, \textcolor{red}{0.31}         & \textcolor{red}{3.17, 0.58}       & \textcolor{blue}{0.41}              \\
% office\_4                       & 2.25, 0.43         & 3.29, 1.03       & \multicolumn{1}{c|}{0.40}              & \textcolor{red}{1.69. 0.32}         & \textcolor{red}{2.50, 0.86}       & \multicolumn{1}{c|}{\textcolor{red}{0.35}}              & 4.84, 0.90         & 24.32, 6.18     & \textcolor{blue}{2.12, 0.41}         & \textcolor{blue}{2.71, 0.96}       & \textcolor{blue}{0.39}              \\ \hline
% \end{tabular}
% \caption{Visual localization results on the Replica dataset. We report median and mean pose error in (cm,\degree), and the sum of L1 distance between predicted scene coordinates and ground truth in $m$. The best and the second best results are labeled to red and blue, respectively.}

% \begin{tabular}{c|ccccccccccc|ccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{11}{c|}{\textbf{Few views training}}                                                                                                                                                & \multicolumn{3}{c}{\textbf{All views training}} \\ \cline{2-15} 
%                                 & \multicolumn{3}{c|}{\textbf{SCRNet}}                 & \multicolumn{3}{c|}{\textbf{SCRNet+ID}}              & \multicolumn{2}{c|}{\textbf{SRC}}             & \multicolumn{3}{c|}{\textbf{Ours}} & \multicolumn{3}{c}{\textbf{SCRNet}}             \\ \cline{2-15} 
%                                 & Median     & Mean       & \multicolumn{1}{c|}{Dist.} & Median     & Mean       & \multicolumn{1}{c|}{Dist.} & Median     & \multicolumn{1}{c|}{Mean}        & Median      & Mean        & Dist.  & Median           & Mean            & Dist.      \\ \hline
% room\_0                         & 2.05, 0.33 & 2.38, 0.36 & \multicolumn{1}{c|}{0.27}  & 2.33, 0.28 & 2.55, 0.32 & \multicolumn{1}{c|}{0.24}  & 2.78, 0.54 & \multicolumn{1}{c|}{3.11, 0.64}  & 1.53, 0.24  & 1.98, 0.27  & 0.22   & 1.84, 0.38       & 2.05, 0.39      & 0.25       \\
% room\_1                         & 1.84, 0.34 & 2.21, 0.42 & \multicolumn{1}{c|}{0.21}  & 1.83, 0.35 & 2.22, 0.42 & \multicolumn{1}{c|}{0.20}  & 1.92, 0.35 & \multicolumn{1}{c|}{3.40, 0.74}  & 1.96, 0.31  & 2.19, 0.38  & 0.17   & 1.99, 0.30       & 2.18, 0.35      & 0.18       \\
% room\_2                         & 1.31, 0.26 & 2.69, 0.65 & \multicolumn{1}{c|}{0.37}  & 1.78, 0.29 & 3.15, 0.69 & \multicolumn{1}{c|}{0.39}  & 2.97, 0.63 & \multicolumn{1}{c|}{13.03, 3.44} & 1.34, 0.22  & 2.57, 0.55  & 0.30   & 1.58, 0.31       & 2.04, 0.49      & 0.35       \\
% office\_0                       & 1.69, 0.34 & 2.01, 0.45 & \multicolumn{1}{c|}{0.17}  & 1.79, 0.37 & 2.24, 0.51 & \multicolumn{1}{c|}{0.19}  & 1.45, 0.30 & \multicolumn{1}{c|}{1.92, 0.43}  & 1.61, 0.35  & 1.97, 0.44  & 0.15   & 1.85, 0.36       & 1.90, 0.42      & 0.15       \\
% office\_1                       & 2.10, 0.52 & 2.23, 0.63 & \multicolumn{1}{c|}{0.34}  & 1.65, 0.42 & 1.99, 0.55 & \multicolumn{1}{c|}{0.26}  & 2.07, 0.53 & \multicolumn{1}{c|}{2.22, 0.59}  & 1.54, 0.44  & 1.74, 0.53  & 0.22   & 1.46, 0.37       & 1.70, 0.45      & 0.30       \\
% office\_2                       & 2.21, 0.41 & 2.54, 0.49 & \multicolumn{1}{c|}{0.29}  & 2.07, 0.37 & 2.28, 0.41 & \multicolumn{1}{c|}{0.27}  & 2.53, 0.51 & \multicolumn{1}{c|}{3.20, 0.64}  & 1.69, 0.33  & 1.93, 0.37  & 0.25   & 2.79, 0.43       & 2.91, 0.44      & 0.28       \\
% office\_3                       & 2.13, 0.37 & 4.91, 0.94 & \multicolumn{1}{c|}{0.44}  & 1.79, 0.28 & 5.72, 1.14 & \multicolumn{1}{c|}{0.40}  & 3.44, 0.63 & \multicolumn{1}{c|}{21.52, 7.95} & 2.40, 0.38  & 4.25, 0.86  & 0.36   & 2.16, 0.31       & 3.17, 0.58      & 0.41       \\
% office\_4                       & 2.25, 0.43 & 3.29, 1.03 & \multicolumn{1}{c|}{0.40}  & 2.42, 0.35 & 3.57, 0.95 & \multicolumn{1}{c|}{0.38}  & 4.84, 0.90 & \multicolumn{1}{c|}{24.32, 6.18} & 1.69. 0.32  & 2.50, 0.86  & 0.35   & 2.12, 0.41       & 2.71, 0.96      & 0.39       \\ \hline
% \end{tabular}
% \caption{result}
% \label{tab:replica_result}
% \end{table*}


% \begin{tabular}{c|ccc|ccc|ccc}
% \hline
% \multirow{2}{*}{\textbf{Scene}} & \multicolumn{3}{c|}{\textbf{SCRNet~\cite{li2020hierarchical} (180 imgs)}}        & \multicolumn{3}{c|}{\textbf{Ours (+150 new views)}}                  & \multicolumn{3}{c}{\textbf{SCRNet~\cite{li2020hierarchical} (All 900 imgs)}}               \\ \cline{2-10} 
%                       & Med.$\downarrow$         & Mean$\downarrow$           & Dist.$\downarrow$ & Med.$\downarrow$         & Mean$\downarrow$           & Dist.$\downarrow$ & Med.$\downarrow$         & Mean$\downarrow$           & Dist.$\downarrow$ \\ \hline
% room\_0                & 2.05, 0.327 & 2.38, 0.363 & 0.270   & 1.53, 0.243 & 1.98, 0.270 & 0.219   & 1.84, 0.379 & 2.05, 0.391 & 0.247   \\
% room\_1                & 1.84, 0.337 & 2.21, 0.424 & 0.207   & 1.96, 0.312 & 2.19, 0.389 & 0.173   & 1.99, 0.296 & 2.18, 0.347 & 0.176   \\
% room\_2                & 1.31, 0.264 & 2.69, 0.654 & 0.373   & 1.34, 0.220 & 2.57, 0.557 & 0.302   & 1.58, 0.309 & 2.04, 0.489 & 0.348   \\
% office\_0              & 1.69, 0.344 & 2.01, 0.445 & 0.171   & 1.61, 0.354 & 1.97, 0.446 & 0.154   & 1.85, 0.356 & 1.90, 0.424 & 0.148   \\
% office\_1              & 2.10, 0.522 & 2.23, 0.631 & 0.338   & 1.54, 0.441 & 1.74, 0.532 & 0.228   & 1.46, 0.372 & 1.70, 0.453 & 0.304   \\
% office\_2              & 2.21, 0.411 & 2.54, 0.489 & 0.286   & 1.69, 0.332 & 1.93, 0.376 & 0.253   & 2.79, 0.427 & 2.91, 0.440 & 0.282   \\
% office\_3              & 2.13, 0.367 & 4.91, 0.939 & 0.443   & 2.40, 0.383 & 4.25, 0.869 & 0.365   & 2.16, 0.313 & 3.17, 0.583 & 0.405   \\
% office\_4              & 2.25, 0.430 & 3.29, 1.030 & 0.397   & 1.69. 0.326 & 2.50, 0.863 & 0.352   & 2.12, 0.405 & 2.71, 0.962 & 0.394   \\ \hline
% \end{tabular}


% \multirow{2}{*}{Scene} & \multicolumn{3}{c}{Available real}         & \multicolumn{3}{c}{Ours}                   & \multicolumn{3}{c}{All real}               \\
%                       & Med.         & Mean           & Distance & Med.         & Mean           & Distance & Med.         & Mean           & Distance \\ \hline
% room\_0                & 0.021, 0.327 & 0.024, 0.363 & 0.270   & 0.015, 0.243 & 0.019, 0.270 & 0.219   & 0.018, 0.379 & 0.021, 0.391 & 0.247   \\
% room\_1                & 0.018, 0.337 & 0.022, 0.424 & 0.207   & 0.019, 0.312 & 0.021, 0.389 & 0.173   & 0.020, 0.296 & 0.022, 0.347 & 0.176   \\
% room\_2                & 0.013, 0.264 & 0.027, 0.654 & 0.373   & 0.013, 0.220 & 0.025, 0.556 & 0.302   & 0.016, 0.309 & 0.020, 0.489 & 0.348   \\
% office\_0              & 0.017, 0.344 & 0.020, 0.445 & 0.171   & 0.016, 0.354 & 0.019, 0.446 & 0.154   & 0.018, 0.356 & 0.019, 0.424 & 0.148   \\
% office\_1              & 0.021, 0.522 & 0.022, 0.631 & 0.338   & 0.015, 0.441 & 0.017, 0.532 & 0.228   & 0.015, 0.372 & 0.017, 0.453 & 0.304   \\
% office\_2              & 0.022, 0.411 & 0.025, 0.489 & 0.286   & 0.017, 0.332 & 0.019, 0.375 & 0.253   & 0.028, 0.427 & 0.029, 0.440 & 0.282   \\
% office\_3              & 0.021, 0.367 & 0.049, 0.939 & 0.443   & 0.024, 0.383 & 0.043, 0.869 & 0.365   & 0.022, 0.313 & 0.032, 0.583 & 0.405   \\
% office\_4              & 0.023, 0.430 & 0.033, 1.030 & 0.397   & 0.017. 0.326 & 0.025, 0.863 & 0.352   & 0.021, 0.405 & 0.027, 0.962 & 0.394   \\ \hline


% \begin{table*}[h]
% \setlength{\abovecaptionskip}{0.3cm}
% \setlength{\belowcaptionskip}{-0.3cm}
% \centering
% % \small
% \footnotesize
% \setlength\tabcolsep{2.6pt}
% \begin{tabular}{c|ccccccccccc|ccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{11}{c|}{\textbf{Few views training}}                                                                                                                                                & \multicolumn{3}{c}{\textbf{All views training}} \\ \cline{2-15} 
%                                 & \multicolumn{3}{c|}{SCRNet~\cite{li2020hierarchical}}                 & \multicolumn{3}{c|}{SCRNet-ID~\cite{ng2021reassessing}}              & \multicolumn{2}{c|}{SRC~\cite{dong2022visual}}             & \multicolumn{3}{c|}{Ours} & \multicolumn{3}{c}{SCRNet~\cite{li2020hierarchical}}             \\ \cline{2-15} 
%                                 & Median$\downarrow$     & Mean$\downarrow$       & \multicolumn{1}{c|}{Dist.} & Median$\downarrow$     & Mean$\downarrow$       & \multicolumn{1}{c|}{Dist.$\downarrow$} & Median$\downarrow$     & \multicolumn{1}{c|}{Mean$\downarrow$}        & Median$\downarrow$      & Mean$\downarrow$        & Dist.$\downarrow$  & Median$\downarrow$           & Mean$\downarrow$            & Dist.$\downarrow$      \\ \hline
% room\_0                         & 2.05, 0.33 & 2.38, 0.36 & \multicolumn{1}{c|}{0.27}  & 2.33, 0.28 & 2.55, 0.32 & \multicolumn{1}{c|}{0.24}  & 2.78, 0.54 & \multicolumn{1}{c|}{3.11, 0.64}  & \textbf{1.53, 0.24}  & \textbf{1.98, 0.27}  & \textbf{0.22}   & 1.84, 0.38       & 2.05, 0.39      & 0.25       \\
% room\_1                         & 1.84, 0.34 & 2.21, 0.42 & \multicolumn{1}{c|}{0.21}  & \textbf{1.83}, 0.35 & 2.22, 0.42 & \multicolumn{1}{c|}{0.20}  & 1.92, 0.35 & \multicolumn{1}{c|}{3.40, 0.74}  & 1.96, \textbf{0.31}  & \textbf{2.19, 0.38}  & \textbf{0.17}   & 1.99, 0.30       & 2.18, 0.35      & 0.18       \\
% room\_2                         & \textbf{1.31}, 0.26 & 2.69, 0.65 & \multicolumn{1}{c|}{0.37}  & 1.78, 0.29 & 3.15, 0.69 & \multicolumn{1}{c|}{0.39}  & 2.97, 0.63 & \multicolumn{1}{c|}{13.0, 3.44} & 1.34, \textbf{0.22}  & \textbf{2.57, 0.55}  & \textbf{0.30}   & 1.58, 0.31       & 2.04, 0.49      & 0.35       \\
% office\_0                       & 1.69, 0.34 & 2.01, 0.45 & \multicolumn{1}{c|}{0.17}  & 1.79, 0.37 & 2.24, 0.51 & \multicolumn{1}{c|}{0.19}  & \textbf{1.45, 0.30} & \multicolumn{1}{c|}{\textbf{1.92, 0.43}}  & 1.61, 0.35  & 1.97, 0.44  & \textbf{0.15}   & 1.85, 0.36       & 1.90, 0.42      & 0.15       \\
% office\_1                       & 2.10, 0.52 & 2.23, 0.63 & \multicolumn{1}{c|}{0.34}  & 1.65, \textbf{0.42} & 1.99, 0.55 & \multicolumn{1}{c|}{0.26}  & 2.07, 0.53 & \multicolumn{1}{c|}{2.22, 0.59}  & \textbf{1.54}, 0.44  & \textbf{1.74, 0.53}  & \textbf{0.22}   & 1.46, 0.37       & 1.70, 0.45      & 0.30       \\
% office\_2                       & 2.21, 0.41 & 2.54, 0.49 & \multicolumn{1}{c|}{0.29}  & 2.07, 0.37 & 2.28, 0.41 & \multicolumn{1}{c|}{0.27}  & 2.53, 0.51 & \multicolumn{1}{c|}{3.20, 0.64}  & \textbf{1.69, 0.33}  & \textbf{1.93, 0.37}  & \textbf{0.25}   & 2.79, 0.43       & 2.91, 0.44      & 0.28       \\
% office\_3                       & 2.13, 0.37 & 4.91, 0.94 & \multicolumn{1}{c|}{0.44}  & \textbf{1.79, 0.28} & 5.72, 1.14 & \multicolumn{1}{c|}{0.40}  & 3.44, 0.63 & \multicolumn{1}{c|}{21.5, 7.95} & 2.40, 0.38  & \textbf{4.25, 0.86}  & \textbf{0.36}   & 2.16, 0.31       & 3.17, 0.58      & 0.41       \\
% office\_4                       & 2.25, 0.43 & 3.29, 1.03 & \multicolumn{1}{c|}{0.40}  & 2.42, 0.35 & 3.57, 0.95 & \multicolumn{1}{c|}{0.38}  & 4.84, 0.90 & \multicolumn{1}{c|}{24.3, 6.18} & \textbf{1.69. 0.32}  & \textbf{2.50, 0.86}  & \textbf{0.35}   & 2.12, 0.41       & 2.71, 0.96      & 0.39       \\ \hline
% \end{tabular}
% \caption{Visual localization results on Replica. We report median and mean  translation and rotation errors (cm,\degree). We also report the sum of the L1 distance between predicted scene coordinates and ground truth in $m$. The best results under the few views training are labeled in bold.}
% \label{tab:replica_result}
% \end{table*}

\begin{table*}[h]
\setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}
\centering
% \small
\scriptsize
\setlength\tabcolsep{3pt}
\begin{tabular}{c|ccccccccccc|ccc}
\hline
\multirow{3}{*}{\textbf{Scene}} & \multicolumn{11}{c|}{\textbf{Few views training}}                                                                                                                                                & \multicolumn{3}{c}{\textbf{All views training}} \\ \cline{2-15} 
                                & \multicolumn{3}{c|}{SCRNet~\cite{li2020hierarchical}}                 & \multicolumn{3}{c|}{SCRNet-ID~\cite{ng2021reassessing}}              & \multicolumn{2}{c|}{SRC~\cite{dong2022visual}}             & \multicolumn{3}{c|}{Ours} & \multicolumn{3}{c}{SCRNet~\cite{li2020hierarchical}}             \\ \cline{2-15} 
                                & Median$\downarrow$     & Mean$\downarrow$       & \multicolumn{1}{c|}{Dist.} & Median$\downarrow$     & Mean$\downarrow$       & \multicolumn{1}{c|}{Dist.$\downarrow$} & Median$\downarrow$     & \multicolumn{1}{c|}{Mean$\downarrow$}        & Median$\downarrow$      & Mean$\downarrow$        & Dist.$\downarrow$  & Median$\downarrow$           & Mean$\downarrow$            & Dist.$\downarrow$      \\ \hline
room\_0                         & 2.05, 0.33 & 2.38, 0.36 & \multicolumn{1}{c|}{0.27}  & 2.33, 0.28 & 2.55, 0.32 & \multicolumn{1}{c|}{0.24}  & 2.78, 0.54 & \multicolumn{1}{c|}{3.11, 0.64}  & \textbf{1.53, 0.24}  & \textbf{1.98, 0.27}  & \textbf{0.22}   & 1.84, 0.38       & 2.05, 0.39      & 0.25       \\
room\_1                         & 1.84, 0.34 & 2.21, 0.42 & \multicolumn{1}{c|}{0.21}  & \textbf{1.83}, 0.35 & 2.22, 0.42 & \multicolumn{1}{c|}{0.20}  & 1.92, 0.35 & \multicolumn{1}{c|}{3.40, 0.74}  & 1.96, \textbf{0.31}  & \textbf{2.19, 0.38}  & \textbf{0.17}   & 1.99, 0.30       & 2.18, 0.35      & 0.18       \\
room\_2                         & \textbf{1.31}, 0.26 & 2.69, 0.65 & \multicolumn{1}{c|}{0.37}  & 1.78, 0.29 & 3.15, 0.69 & \multicolumn{1}{c|}{0.39}  & 2.97, 0.63 & \multicolumn{1}{c|}{13.0, 3.44} & 1.34, \textbf{0.22}  & \textbf{2.57, 0.55}  & \textbf{0.30}   & 1.58, 0.31       & 2.04, 0.49      & 0.35       \\
office\_0                       & 1.69, 0.34 & 2.01, 0.45 & \multicolumn{1}{c|}{0.17}  & 1.79, 0.37 & 2.24, 0.51 & \multicolumn{1}{c|}{0.19}  & \textbf{1.45, 0.30} & \multicolumn{1}{c|}{\textbf{1.92, 0.43}}  & 1.61, 0.35  & 1.97, 0.44  & \textbf{0.15}   & 1.85, 0.36       & 1.90, 0.42      & 0.15       \\
office\_1                       & 2.10, 0.52 & 2.23, 0.63 & \multicolumn{1}{c|}{0.34}  & 1.65, \textbf{0.42} & 1.99, 0.55 & \multicolumn{1}{c|}{0.26}  & 2.07, 0.53 & \multicolumn{1}{c|}{2.22, 0.59}  & \textbf{1.54}, 0.44  & \textbf{1.74, 0.53}  & \textbf{0.22}   & 1.46, 0.37       & 1.70, 0.45      & 0.30       \\
office\_2                       & 2.21, 0.41 & 2.54, 0.49 & \multicolumn{1}{c|}{0.29}  & 2.07, 0.37 & 2.28, 0.41 & \multicolumn{1}{c|}{0.27}  & 2.53, 0.51 & \multicolumn{1}{c|}{3.20, 0.64}  & \textbf{1.69, 0.33}  & \textbf{1.93, 0.37}  & \textbf{0.25}   & 2.79, 0.43       & 2.91, 0.44      & 0.28       \\
office\_3                       & 2.13, 0.37 & 4.91, 0.94 & \multicolumn{1}{c|}{0.44}  & \textbf{1.79, 0.28} & 5.72, 1.14 & \multicolumn{1}{c|}{0.40}  & 3.44, 0.63 & \multicolumn{1}{c|}{21.5, 7.95} & 2.40, 0.38  & \textbf{4.25, 0.86}  & \textbf{0.36}   & 2.16, 0.31       & 3.17, 0.58      & 0.41       \\
office\_4                       & 2.25, 0.43 & 3.29, 1.03 & \multicolumn{1}{c|}{0.40}  & 2.42, 0.35 & 3.57, 0.95 & \multicolumn{1}{c|}{0.38}  & 4.84, 0.90 & \multicolumn{1}{c|}{24.3, 6.18} & \textbf{1.69. 0.32}  & \textbf{2.50, 0.86}  & \textbf{0.35}   & 2.12, 0.41       & 2.71, 0.96      & 0.39       \\ \hline
\end{tabular}
\caption{Visual localization results on Replica. We report median and mean  translation and rotation errors (cm,\degree). We also report the sum of the L1 distance between predicted scene coordinates and ground truth in $m$. The best results under the few views training are labeled in bold.}
\label{tab:replica_result}
\vspace{-0.4cm}
\end{table*}

% \vspace{-3cm}

% \begin{table*}[]
% \setlength{\abovecaptionskip}{0.2cm}
% % \setlength{\belowcaptionskip}{-0.5cm}
% \centering
% % \small
% \footnotesize
% \setlength\tabcolsep{2.6pt}
% \begin{tabular}{c|ccccccccccc|ccc}
% \hline
% \multirow{3}{*}{\textbf{Scene}} & \multicolumn{11}{c|}{\textbf{Few views training}}                                                                                                                                                & \multicolumn{3}{c}{\textbf{All views training}} \\ \cline{2-15} 
%                                 & \multicolumn{3}{c|}{\textbf{SCRNet~\cite{li2020hierarchical}}}                 & \multicolumn{3}{c|}{\textbf{SCRNet+ID~\cite{ng2021reassessing}}}              & \multicolumn{2}{c|}{\textbf{SRC~\cite{dong2022visual}}}             & \multicolumn{3}{c|}{\textbf{Ours}} & \multicolumn{3}{c}{\textbf{SCRNet~\cite{li2020hierarchical}}}             \\ \cline{2-15} 
%                                 & Median$\downarrow$     & Mean$\downarrow$       & \multicolumn{1}{c|}{Dist.} & Median$\downarrow$     & Mean$\downarrow$       & \multicolumn{1}{c|}{Dist.$\downarrow$} & Median$\downarrow$     & \multicolumn{1}{c|}{Mean$\downarrow$}        & Median$\downarrow$      & Mean$\downarrow$        & Dist.$\downarrow$  & Median$\downarrow$           & Mean$\downarrow$            & Dist.$\downarrow$      \\ \hline
% room\_0                         & 2.05, 0.33 & 2.38, 0.36 & \multicolumn{1}{c|}{0.27}  & 2.33, 0.28 & 2.55, 0.32 & \multicolumn{1}{c|}{0.24}  & 2.78, 0.54 & \multicolumn{1}{c|}{3.11, 0.64}  & \textbf{1.53, 0.24}  & \textbf{1.98, 0.27}  & \textbf{0.22}   & 1.84, 0.38       & 2.05, 0.39      & 0.25       \\
% room\_1                         & 1.84, 0.34 & 2.21, 0.42 & \multicolumn{1}{c|}{0.21}  & \textbf{1.83}, 0.35 & 2.22, 0.42 & \multicolumn{1}{c|}{0.20}  & 1.92, 0.35 & \multicolumn{1}{c|}{3.40, 0.74}  & 1.96, \textbf{0.31}  & \textbf{2.19, 0.38}  & \textbf{0.17}   & 1.99, 0.30       & 2.18, 0.35      & 0.18       \\
% room\_2                         & \textbf{1.31}, 0.26 & 2.69, 0.65 & \multicolumn{1}{c|}{0.37}  & 1.78, 0.29 & 3.15, 0.69 & \multicolumn{1}{c|}{0.39}  & 2.97, 0.63 & \multicolumn{1}{c|}{13.0, 3.44} & 1.34, \textbf{0.22}  & \textbf{2.57, 0.55}  & \textbf{0.30}   & 1.58, 0.31       & 2.04, 0.49      & 0.35       \\
% office\_0                       & 1.69, 0.34 & 2.01, 0.45 & \multicolumn{1}{c|}{0.17}  & 1.79, 0.37 & 2.24, 0.51 & \multicolumn{1}{c|}{0.19}  & \textbf{1.45, 0.30} & \multicolumn{1}{c|}{\textbf{1.92, 0.43}}  & 1.61, 0.35  & 1.97, 0.44  & \textbf{0.15}   & 1.85, 0.36       & 1.90, 0.42      & 0.15       \\
% office\_1                       & 2.10, 0.52 & 2.23, 0.63 & \multicolumn{1}{c|}{0.34}  & 1.65, \textbf{0.42} & 1.99, 0.55 & \multicolumn{1}{c|}{0.26}  & 2.07, 0.53 & \multicolumn{1}{c|}{2.22, 0.59}  & \textbf{1.54}, 0.44  & \textbf{1.74, 0.53}  & \textbf{0.22}   & 1.46, 0.37       & 1.70, 0.45      & 0.30       \\
% office\_2                       & 2.21, 0.41 & 2.54, 0.49 & \multicolumn{1}{c|}{0.29}  & 2.07, 0.37 & 2.28, 0.41 & \multicolumn{1}{c|}{0.27}  & 2.53, 0.51 & \multicolumn{1}{c|}{3.20, 0.64}  & \textbf{1.69, 0.33}  & \textbf{1.93, 0.37}  & \textbf{0.25}   & 2.79, 0.43       & 2.91, 0.44      & 0.28       \\
% office\_3                       & 2.13, 0.37 & 4.91, 0.94 & \multicolumn{1}{c|}{0.44}  & \textbf{1.79, 0.28} & 5.72, 1.14 & \multicolumn{1}{c|}{0.40}  & 3.44, 0.63 & \multicolumn{1}{c|}{21.5, 7.95} & 2.40, 0.38  & \textbf{4.25, 0.86}  & \textbf{0.36}   & 2.16, 0.31       & 3.17, 0.58      & 0.41       \\
% office\_4                       & 2.25, 0.43 & 3.29, 1.03 & \multicolumn{1}{c|}{0.40}  & 2.42, 0.35 & 3.57, 0.95 & \multicolumn{1}{c|}{0.38}  & 4.84, 0.90 & \multicolumn{1}{c|}{24.3, 6.18} & \textbf{1.69. 0.32}  & \textbf{2.50, 0.86}  & \textbf{0.35}   & 2.12, 0.41       & 2.71, 0.96      & 0.39       \\ \hline
% \end{tabular}
% \caption{Visual localization results on the Replica dataset. We report median and mean pose error in (cm, \degree), and the sum of L1 distance between predicted scene coordinates and ground truth in $m$. The best results under the few views training are labeled in bold.}
% \label{tab:replica_result}
% \end{table*}
